ChartText: Linking Text with Charts in Documents

Recent works show that interactive documents connecting text with visualizations facilitate reading comprehension. However, creating this type of content requires specialized knowledge. We present ChartText, a method that links text with visualizations in this work. Our approach supports documents that include bar charts, line charts, and scatter plots. ChartText receives the visual encoding of the visualization and its associated text as input. It then performs the linking in two stages: The matching stage creates individual links relating simple phrases between the text and the chart. Then, it combines the individual links according to the visual channels in the grouping stage, building more meaningful connections. We use two datasets to design and evaluate our method; the first comes from web documents (24 bar charts and texts) and the second from academic documents (25 bar charts, 25 line charts, and 25 scatter plots with their texts). Our experiments show that our method obtains F1 scores of 0.50 and 0.66 on both datasets. We can also use a semi-automatic approach correcting individual links; in this case, the scores rise to 0.68 and 0.84, respectively. To show the usefulness of our technique, we implement two proofs of concept. We create interactive documents using graphic overlays in the first one, facilitating the reading experience. We use voice instead of text to annotate charts in real-time in the second. For example, in a videoconference, our technique can automatically annotate a chart following the presenter's description.

==> Makefile <==
# --------------------------------------------------------------------
# Usage:
#
#	all	 make pdf file
#	pdf	 make pdf file
#	clean	 remove files
#	clobber  remove everything
#	check	 doubled word and latex syntax check
#	wc	 word count
# --------------------------------------------------------------------

NAME := paper
BIBFILES := paper.bib
TEXFILES := paper.tex

DISTILLER := ps2pdf

# --------------------------------------------------------------------

SHELL := bash
LATEX := pdflatex
BIBTEX := bibtex -min-crossrefs=100 # avoid separating out crossrefs
DETEX := detex -n
LACHECK := lacheck
DW := dw # ftp://ftp.math.utah.edu/pub/misc/dw.tar.gz
RM := rm -f
WC := wc

# --------------------------------------------------------------------

all: $(NAME).pdf 
pdf: $(NAME).pdf
check: dw syn

$(NAME).pdf: $(NAME).tex $(BIBFILES) 
	@echo '-------------------- latex appendix --------------'
	#$(LATEX) appendix.tex
	#$(BIBTEX) appendix
	#$(LATEX) appendix.tex
	#$(LATEX) appendix.tex
	@echo '-------------------- latex #1 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- bibtex --------------------'
	$(BIBTEX) $(NAME)
	@echo '-------------------- latex #2 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- latex #3 --------------------'
	$(LATEX) $(NAME).tex

dw:
	@-$(RM) $(NAME).dw
	@echo '-------------------- doubled words --------------------'
	@for f in $(NAME).tex ;\
	do \
		echo ----- $$f ----- ; \
		echo ----- $$f ----- >> $(NAME).dw ; \
		$(DETEX) $$f  | $(DW) >> $(NAME).dw ; \
	done

syn:
	@echo '-------------------- syntax check --------------------'
	@$(LACHECK) $(NAME).tex

wc:
	@$(DETEX) $(NAME).tex | $(WC)

clean:
	$(RM) *.{blg,dvi,dw,ilg,log,o,tmp,lbl,aux,bbl,lbl}
	$(RM) *.{idx,ind,toc,lof,lot,brf,out,fls,fdb_latexmk,synctex.gz}
	$(RM) $(NAME).pdf

clobber: clean
	$(RM) *~ \#* core


==> related.tex <==
\section{Related work}
Our work relates to two main areas: (i) chart interpretation and (ii) techniques and applications to facilitate the reading of documents.

% \subsection{Text-to-Image Coreference Resolution}
% This field consists of predicting the region of an image that corresponds to automatically-identified entities in the text (\eg, objects, people, and locations).
% %
% Initially, this task arises from the need to improve caption-generating systems.
% %
% One of the first to perform this task is the work of Kong~et~al.~\cite{what_are_you_talkin_about}.
% %
% This work shows that it is possible to improve the captions of 3D scenes, describing the objects in the scene separately.
% %
% The authors train a Markov Random Field model~\cite{sherman1973markov} that learns the correspondence between text entities and scene objects.
% %
% Then, they analyze the POS (Part Of Speech) tags to identify properties of the entities in the text associated with the objects (\ie, color, size, and position).
% %
% Finally, they use the properties to enhance the caption.
% %
% Later, Plummer~et~al.~\cite{Plummer2015} presents a semi-automatic process to build a dataset containing annotations for this task.
%
% The dataset extends Young~et~al.~\cite{young-etal-2014-image} that originally included images and their natural language descriptions to generate captions.
% %
% They validate their new dataset by training a Canonical Correlation Analysis model~\cite{darlington1973canonical} for the text-to-image coreference resolution task.
% %
% The model is capable of representing an image and a text in the same semantic space.
% %
% Taking advantage of this representation, it is possible to relate the images and the text using strategies such as cosine distance to decide a correspondence.
% %
% This approach has some limitations since the model does not consider the semantic relationships among entities in the sentence.
% %
% By not considering the semantics relationship among entities, it can erroneously associate a region in the image with an entity in the text. This mistake occurs when the entity appears more than once in the sentence.
% %
% To solve this problem, Wang~et~al.~\cite{Wang2016} applies restriction when two entities have a semantic relationship, making their corresponding regions have a visual relationship that is consistent with the semantic relationship.
% %
% Despite the improvements in this field, there is not much data tagged to train models to perform this task. In response, Rohrbach~et~al.~\cite{Rohrbach2016} uses unsupervised training and attention mechanisms to generate bounding boxes of the image regions that relate to entities in the sentences. However, it is still necessary an extensive set of images and sentence data to perform the training.
%
%
% The task of relating entities of a text to regions of the image is very similar to our primary objective. However, we focus on documents that contains data-driven visualizations, rather than natural images. This means that there are limitations to using approaches similar to those reviewed to solve our problem. The main limitation is related to the small amount of data annotated to train a sophisticated detection model. In this paper, we propose a rule-based method to address the problem and serve as a starting point for future research.


\subsection{Chart Interpretation}
In recent years, methods and techniques have been developed to automatically extract the underlying data and visual encoding that build up charts.
%
These techniques have applications such as the reuse and redesign of charts. One of the pioneers in this area is ReVision~\cite{savva2011revision}. 
%
ReVision extracts the data that generates a visualization from an image in a bitmap format.
%
ReVision proposes a pipeline where initially the images are classified using the Support Vector Machine model~\cite{SVMHearst1998} to determine the type of chart (\ie, bar chart, line chart, and scatter plot).
%
Then, they use different image processing techniques and heuristics. These methods are adapted to the type of chart and then used to filter elements in the image and identify the data.
%
Other works maintain the initial idea of ReVision but vary some components with more sophisticated models. For instance, FigureSeer~\cite{siegel2016figureseer} and Scatterract~\cite{cliche2017scatteract} use a Convolutional Neural Network~\cite{cnnlecun}. 
%
The input of these systems consists of images and features based on the spatial information of the chart elements to enhance the classification task. 
%
They also take advantage of the axis information and text labels to infer the data on line charts and scatter plots, respectively. 
%
Later, ChartSense~\cite{jung2017chartsense} extended the data extraction support for five chart types (line chart, bar chart, area chart, foot chart, and radar chart), diversifying the heuristics to extract the data for each chart type but keeping the main idea proposed in previous works.


Other work focuses on recovering the visual encoding of the chart. 
%
For instance, Harper et al.~\cite{harper2014deconstructing} developed a system to deconstruct visualizations created with the D3~library~\cite{bostock2011d3}.
%
This technique uses the data and graphic elements, which are easier to access in SVG images, to compose the visual encoding. In the same vein, Poco and Heer~\cite{poco2017reverse} propose a pipeline to recover the visual encoding but for bitmap images.
%
The technique exploits only the textual elements and retrieves a visual encoding in a declarative language similar to Vega-Lite~\cite{satyanarayan2017vega}. 
%
Later, Chen et al.~\cite{chen2019towards} present a method to deconstruct bitmap infographics and generate templates that can be reused to create new infographics. 
%
This method uses deep learning models to identify graphics elements. 
%
Although we do not deconstruct charts in our work, we assume that we have the visual encoding as input. This assumption is valid since we can create visual encoding using any of the methods described above.



\subsection{Facilitating the Reading of Documents}
Recently many works have appeared in this line. 
Kong and Agrawala~\cite{kong2012graphical} introduce Graphical Overlays to create interactive charts by accessing the data and visual encoding (using ReVision~\cite{savva2011revision}). 
%
We also have a similar application; however, we generate overlays based on the text accompanying a chart; in this sense, our goal is to facilitate document reading. 

\change{
Other works take advantage of additional information that is accessible to enrich documents and visualizations. For instance, Metoyeret et al.~\cite{coupling-story} present a technique that works on data-rich stories (\ie, texts with access to additional data such as tables). They propose using text analysis to connect narrative sentences with visual elements that describe the rich data. Bryan et al.~\cite{temporal-summ} propose a method to explore temporal data and find, through heuristics, points of interest in the data that allow the creation of explanatory visualizations. Hullman et al.~\cite{Contextifier} propose a system that takes time series data on a company's stock to automatically create a line chart enriched with annotations from text analysis and metadata from news articles related to the company. These approaches are helpful when we have access to the data that accompanies the document or visualization. However, we only need the chart texts available in the visual encoding and easy to extract with fewer errors in our approach.
}


Later, Kong et al.~\cite{kong2014extracting} presented a crowdsourcing-based method for extracting links between charts and text in documents. 
%
Nevertheless, they use people to annotate the document using crowdsourcing, unlike our work, which is fully automatic.
%
On the other hand, there are works that, instead of using visualizations, use tables. 
%
Kim et al.~\cite{kim2018facilitating} presented an automatic technique to find links between tables and paragraphs. 
%
This work uses NLP and heuristic techniques to connect table cells with text sentences. 
%
Similarly, Badam et al.~\cite{Badam2018ElasticDC} proposed a web tool that relates the text to the tables and creates visualizations using these links. 
%
To reduce the effort to create interactive documents, Latif et al.~\cite{linkingfra} proposed a framework for systematically generating documents that support text-visualization interaction. 
%
This system allows users to annotate the links in a declarative language. 
%
Then, Cui et al.~\cite{Cui2019TexttoVizAG} proposed a method that converts text into infographics to facilitate reading. First, they identify parts of the text that refer to some data (\eg, numbers) and then use this information in templates that generate the image.
%
Later, Latif et al.~\cite{s.20191180} presented an approach for producing interactive documents for graph data, also using a declarative syntax that requires little to no programming skills. 
%
Recently, Lai et al.~\cite{autoannotation} proposed a system with similar capabilities. 
%
Nevertheless, there are two significant differences: First, they use short textual descriptions tied to visual elements in the chart. 
%
For instance, the phrase \phrase{the red point} in the context of a scatter plot refers to the graphical mark “point” and the legend label \phrase{red.} Our work identifies textual descriptions related to a narrative aspect of the visualization; for instance, \phrase{the oracle achieves 96.23\% when k=10}. 
%
In other words, they focus only on individual links; in our case, we have a second stage grouping the individual link to make more meaningful associations.
%
Second, Lait et al. require access to the encoded data, whereas our technique only requires the textual elements, representing a more straightforward task and less prone to error.



